Dynamic Flow Scheduling Strategy in Multihoming Video CDNs

Multihoming for a video Content Delivery Network (CDN) allows edge peering servers to deliver video chunks through different Internet Service Providers (ISPs), to achieve an improved quality of service (QoS) for video streaming users. However, since traditional strategies for a multihoming video CDN are simply designed according to static rules, e.g., simply sending traffic via a ISP which is the same as the ISP of client, they fail to dynamically allocate resources among different ISPs over time. In this paper, we perform measurement studies to demonstrate that such static allocation mechanism is inefficient to make full utilization of multiple ISPs' resources. To address this problem, we propose a dynamic flow scheduling strategy for multihoming video CDN. The challenge is to find the control parameters that can guide the ISP selection when performing flow scheduling. Using a data-driven approach, we find factors that have a major impact on the performance improvement in the dynamic flow scheduling. We further utilize an information gain approach to generate parameter combinations that can be used to guide the flow scheduling, i.e., to determine the ISP each request should be responded by. Our evaluation results demonstrate that our design effectively performs the flow scheduling. In particular, our design yields near optimal performance in a simulation of real-world multihoming setup.

==> sections/backgroundmotivation.tex <==
\section{Background and Motivation}

\subsection{Multiple ISP Portal Datacenter}
%Most of the materials is the configuration of router for load-balance 
%DSN load balancer
%Cisco: ios NAT load-balancing for two isp connections
\subsection{Problems of Today's Schedule}
%目前用于服务边缘用户的的数据中心以及CDN站点
\subsubsection{OSPF Problem}
 OSPF protocol only concentrating on the flow that it is transfering lacks of global perspective and takes no account of other flows. The OSPF cost setting have an influence on the shortest path selection between the servers and the clients. In reality, we assume the topolgy of the network are steady for a  period, then OSPF has a determinate link cost as its basic routing metric. For instance,Cisco router set the cost like $10^8/bandwidth$ by default.Many proposals extended OSPF protocol through optimizing the algorithms of selecting link weight or adding the operation of splitting flows in many paths.
%ISP内部OSPF采用固定的cost设置网络收敛后很长时间内网络路径不会变化，使网络没有很好的动态特性，导致网络拥塞，单点失效造成的网络瘫痪等事件的出现。OSPF根据带宽的倒数来计算接口的OSPF度量值，在CISCO路由器中，成本=100Mbits/BW
\subsubsection{Manually Schedule Problem}
%有些关于带宽优化的算法计算量大且需要ISP内部进行配置，不够实际ISP不配合。
\subsubsection{Problems of Previous Approaches}
%原来的部署困难，花费大

\subsection{The Potential of First-Hop SDN/Scheduler/ Proxy}
In our CDN-SDN hybrid network, we assume that the SDN nodes is the direct connecting switch to CDN sites, It can centrally control the clients flows and ensure the diffrent first hops selection for diffrent clients.We conduct the experiments to show that we can reap a nice benefit if we only deploy SDN nodes on the export of CDN sites. 
%SDN流量分配，CDN第一跳将搜集网络信息，扰动起来
\subsubsection{Under Different Topologies}

\subsubsection{Under Different Network Scale}



\subsection{Factors that Affect the Performance of First-Hop SDN Scheme}

==> sections/discussion.tex <==
\section{Practical Issues Discussion}
 \label{sec:Implementation}
 
In this section, we explore some practical issues to answer the question: how do CDN providers utilize our study results to improve their content delivery performance? Although content distribution involves a complex ecosystem consisting of many parties, i.e., clients, CDNs and ISPs, our flow scheduling strategy is a feasible solution since its deployment only depends on CDNs.

\subsection{Implementation Framework}
 \begin{figure}[t]
	\begin{minipage}[t]{\linewidth}
    \centering
    \includegraphics [width=\linewidth]{5-1scheme.pdf}
  	\end{minipage}
 	\hfill
  \caption{The framework of dynamic flow scheduling.}
  \label{fig:The framework of dynamic flow scheduling.}
\end{figure}

Fig. \ref{fig:The framework of dynamic flow scheduling.} illustrates an implementation framework of our flow scheduling design. Network information updater contains a database with all of the IPs needed to be traced. For each update time slot, it renews the network information databases, including the topology paths from the peering server to each client network (network topology database), and the bottleneck information (network dynamics database). 

Flow scheduling decision maker maintains two important hash tables, hash table 1 and hash table 2. Hash table 1 associates the client networks to its corresponding outgoing ISPs. Hash table 2 associates the parameters (i.e., $E_{k}$, $O_{k}$ and $W_{k}$) to the flow scheduling strategy $k$. Hash table 1 updates according to hash table 2, which is calculated according to the network information database.

When a client initiates a request for a video file, two actions are invoked at the peering server:
\begin{itemize}
\item The flow scheduling decision maker checks whether this client network has a corresponding entry in hash table 1. If there is an entry for this client network, our scheme returns a video chunks with the proper outgoing ISP. Otherwise, the request is responded through an default outgoing ISP (e.g., the same ISP with the client). 
\item The IP sampler decides whether to trace this client IP. If this IP belongs a client network we never know or its client network information needs to be updated, the IP sampler adds this client IP to the database of network information updater with 60\% chance.
\end{itemize}
 
 	
\subsection{The Acquisition of the Parameters}


\textbf{Network Topology Information for Network Topology Database.} We utilize Traceroute to discover the routing paths from peering server to client networks. The parameters $E_{k}$ and $O_{k}$ can be calculated from the path information. These two parameters are not necessary to be updated with a high frequency because the network topology is stationary for at least a finite period of time \cite{Paxson:1997:ERB:268715.268716}. In our design, we probe the client networks every day.


\textbf{Network Dynamics Information for Network Dynamics Database.} In our design, we allow CDN edge sites to obtain the network dynamics information by Pathneck, an available bandwidth measurement tool that is suitable for our design. Pathneck is an active probing tool that can detect bottlenecks, both of its locations and upper available bandwidth bounds, with a relatively small probing overhead (33.6KB for one probing in the default setting) and a fast probe speed (average $2.5$s for one probing in our actual measurement). Moreover, Pathneck is an single-end probe tool that can be implemented by the CDN sites alone. Parameter $W_{k}$ is calculated from the information provided from Pathneck. Bottleneck information needs a higher frequency probe rate than routing paths due to the network traffic dynamics. We carry out Pathneck trace each hour during non-peak usage times and every 30 min during peak usage times in order to update the flow scheduling strategy timely.

Selecting the ISP to serve a client network depends on the time-varying parameters for each flow scheduling strategy. We set IP Sampler to only trace $60$\% of the client networks and all of the parameters are traced on the CDN edge sites. It is also redundant to trace path information for each client IP from the same client network. Because most of these client IPs follow the same path from the CDN edge site to the same stub network \cite{lee2004exploiting}. Then a small set of clients (e.g., three clients) in each client network is randomly chosen as the probe targets in our design.
 
 
  
\subsection{Real-world Deployment}

Two main solutions are available to deploy multihoming technology in CDNs in order to deliver the video with the proper outgoing ISP, NAT-multihoming \cite{NATMultihoming} and BGP-multihoming \cite{BGPmultihoming}. We use the BGP-multihoming as our example and analyze how BGP-multihoming CDNs integrate with our dynamic flow scheduling strategy. Controlling the outbound ISP at a peering CDN site needs to consider two conditions. 

First, the CDN site has its own independent address block \cite{liu2007survey}. A large CDN provider may apply for a IP address block directly from an independent authority, e.g., Asia Pacific Network Information Centre (APNIC). In this case, to enable intelligent outgoing ISPs selection, the conventional way is that the border routers of the CDNs apply certain routing policies in the BGP path selection, e.g., appropriately setting LOCAL PREFERENCE \cite{BGPR} attribute to the router over time, to actively schedule flows. 

Second, the CDN site has assigned address from its upstream ISPs, i.e., CDN site has the sub-network IP address blocks of each its upstream ISPs. Due to security or some other commercial reasons, upstream ISPs may refuse to accept traffic from the CDN sites with a source address prefix that is not advertised to this ISP by the CDN network. Then the CDN providers could rely on the DNS to select a peering server that connects the right outgoing ISP. When DNS resolver receives a video request, it determines which peering server to choose with the IP that can be routed by a specific ISP. Other technologies like HTTP redirection and client-tailored HTML rewriting are also off-the-peg methods to implement the flow scheduling strategy.
  
 The implementation of flow scheduling based on BGP is inflexible to install a mass of routing rules, and DNS-based method may lead to the start delay along with the DNS-based method. Then we consider a newer technology, SDN. SDN is an innovation network architecture that attracts research attention in recent years. SDX \cite{Gupta:2014:SSD:2619239.2626300} integrates Software Defined Network (SDN) and BGP. It indicates that the programmatic integration of flow scheduling and BGP might be less costly in the future. SDN techniques can be exploited to direct the different flows to the same destination through different ISPs. We can deploy a SDN router at the outgoing points of CDN sites. When the server receives a video request, CDN-SDN controller calculates the best outgoing ISP by our local selection flow scheduling algorithms and installs the rule in SDN router. We believe this CDN-SDN hybrid solution is a potential way.
   
 %\textbf{Selecting outgoing ISPs over NAT-multihoming technology.} %Akella et al. \cite{4444747} discussed the implementation of flow scheduling by NAT/DNS based method.The essential function of the DNS-based techniques is to provide the address of the "appropriate" interface for each arriving client. 
 
 %\textbf{Selecting outgoing ISPs over BGP-multihoming technology.} 
 %When a CDN site is connected to multiple ISPs, CDN AS will likely receive multiple route announcements to a given destination network prefix, of which the CDN AS selects the best route based on policy and other considerations.
 
 % ToN 用代理的方法实现了出口路径选择
 %\cite{4444747} BGP和SDN共存，很好的使不同用户install不同的出口规则，我们未来考虑实现SDN-CDN结合，为NFV网络虚拟化进程的加快做出贡献。


 %Nowadays, tens of thousands of clients served by even only one CDN server. So performing traceroute or Pathneck probes to each clients via each ISPs of multihoming CDN is unrealistic. In order to reduce to cost and improve the scalability of information collection, we carry out a measurement-based study to analyze the reduction of the probes. We extract all of the  client IP addresses from a client video streaming demands' log from BesTv. then sample it by the network prefixes. From each prefix, we randomly select five IP addresses and conducted a experiments to collect traceroute data to these client IPs via the two-multihomed servers in Sec. \ref{sec:real-world}. Based on the traceroute data, we discover paths to many clients in the same customer network follow the same path over the same outgoing ISPs. Then we translate an IP to a geo-location and cluster the clients by tuple (ISP/IP prefix, location), We can sample a few clients.







 

